AdsorbML: A Leap in Efficiency for Adsorption Energy Calculations using Generalizable Machine Learning Potentials

Computational catalysis is playing an increasingly significant role in the design of catalysts across a wide range of applications. A common task for many computational methods is the need to accurately compute the adsorption energy for an adsorbate and a catalyst surface of interest. Traditionally, the identification of low energy adsorbate-surface configurations relies on heuristic methods and researcher intuition. As the desire to perform high-throughput screening increases, it becomes challenging to use heuristics and intuition alone. In this paper, we demonstrate machine learning potentials can be leveraged to identify low energy adsorbate-surface configurations more accurately and efficiently. Our algorithm provides a spectrum of trade-offs between accuracy and efficiency, with one balanced option finding the lowest energy configuration 87.36% of the time, while achieving a 2000x speedup in computation. To standardize benchmarking, we introduce the Open Catalyst Dense dataset containing nearly 1,000 diverse surfaces and 100,000 unique configurations.

==> tables/ml_only_success.tex <==
\begin{table*}[h]
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Success Rate} [\%] $\uparrow$} & \multirow{2}{*}{\textbf{$\Delta$ E} {[}eV{]}} \\ \cmidrule(lr){2-3}
                   & Unvalidated & Validated &         \\ \midrule
SchNet             & 36.49\% & 1.44\%       & -9.8745 \\
DimeNet++          & 57.76\% & 2.57\%       & -1.2018 \\
PaiNN              & 72.35\% & 12.54\%      & -0.3374 \\
GemNet-OC          & 80.68\% & 42.75\%      & -0.1276 \\
GemNet-OC-MD       & 77.49\% & 41.11\%      & -0.1196 \\
GemNet-OC-MD-Large & 79.96\% & 45.43\%      & -0.0787 \\
SCN-MD-Large       & 81.91\% & 50.36\%      & -0.0814 \\ \bottomrule
\end{tabular}%
}
\caption{A comparison of ML success rates with and without \gls{DFT} validation. An ML system is considered validated if it's predicted energy is within 0.1 eV of a corresponding \gls{DFT} evaluation of that structure. The large gap between the two success metrics suggests \gls{ML} energies are highly optimistic and should not be blindly trusted.\label{tab:ml-only-success}}
\end{table*}

==> tables/val_breakdown.tex <==
% Validation
\begin{table*}[ht]
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\multicolumn{7}{c}{Success Rate} \\ \midrule
\multicolumn{7}{c}{DFT single-point on ML relaxed structures (ML+SP)} \\ \midrule
 & \multicolumn{3}{c|}{\textit{k=1}} & \multicolumn{3}{c}{\textit{k=5}} \\
\textbf{Model} & \multicolumn{1}{l}{Much better} & Parity & \multicolumn{1}{c|}{Much worse} & Much better & Parity & Much worse \\
SchNet & 0.62\% & 2.16\% & \multicolumn{1}{c|}{97.23\%} & 1.03\% & 4.01\% & 94.96\% \\
DimeNet++ & 1.44\% & 3.91\% & \multicolumn{1}{c|}{94.66\%} & 3.91\% & 6.89\% & 89.21\% \\
PaiNN & 3.80\% & 23.64\% & \multicolumn{1}{c|}{72.56\%} & 5.04\% & 34.53\% & 60.43\% \\
GemNet-OC & 5.96\% & 62.80\% & \multicolumn{1}{c|}{31.24\%} & 11.82\% & 71.12\% & 17.06\% \\
GemNet-OC-MD & 7.81\% & 60.95\% & \multicolumn{1}{c|}{31.24\%} & 15.52\% & 68.86\% & 15.62\% \\
GemNet-OC-MD-Large & 6.27\% & 66.91\% & \multicolumn{1}{c|}{26.82\%} & 8.53\% & 77.49\% & 13.98\% \\
SCN-MD-Large & 5.76\% & 72.05\% & \multicolumn{1}{c|}{22.20\%} & 7.40\% & 80.37\% & 12.23\% \\ \midrule
\multicolumn{7}{c}{DFT relaxations on ML relaxed structures (ML+RX)} \\ \midrule
 & \multicolumn{3}{c|}{\textit{k=1}} & \multicolumn{3}{c}{\textit{k=5}} \\
\textbf{Model} & Much better & Parity & \multicolumn{1}{c|}{Much worse} & Much better & Parity & Much worse \\
SchNet & 3.70\% & 31.55\% & \multicolumn{1}{c|}{64.75\%} & 7.91\% & 50.15\% & 41.93\% \\
DimeNet++ & 3.60\% & 39.88\% & \multicolumn{1}{c|}{56.53\%} & 12.13\% & 55.81\% & 32.07\% \\
PaiNN & 5.65\% & 56.01\% & \multicolumn{1}{c|}{38.34\%} & 10.48\% & 70.71\% & 18.81\% \\
GemNet-OC & 6.17\% & 67.42\% & \multicolumn{1}{c|}{26.41\%} & 13.36\% & 76.05\% & 10.59\% \\
GemNet-OC-MD & 8.02\% & 64.23\% & \multicolumn{1}{c|}{27.75\%} & 16.03\% & 72.46\% & 11.51\% \\
GemNet-OC-MD-Large & 6.47\% & 69.68\% & \multicolumn{1}{c|}{23.84\%} & 9.76\% & 79.14\% & 11.10\% \\
SCN-MD-Large & 5.04\% & 75.54\% & \multicolumn{1}{c|}{19.42\%} & 8.22\% & 82.43\% & 9.35\% \\ \bottomrule
\end{tabular}
}
\caption{\label{tab:breakdowns}Distribution of success rates for the proposed ML+SP and ML+RX strategies. ``Parity" corresponds to being within 0.1 eV of the \gls{DFT} adsorption energy; ``Much better" corresponds to being less than 0.1 eV than \gls{DFT}; and ``Much worse" being higher than 0.1 eV of \gls{DFT}. Due to constraint filtering, it is possible that ML+SP results may be higher than ML+RX results in some cases (e.g. SCN-MD-Large).}
\end{table*}
